Convergence of a low-rank Lie--Trotter splitting for stiff matrix differential equations

We propose a numerical integrator for determining low-rank approximations to solutions of large-scale matrix differential equations. The considered differential equations are semilinear and stiff. Our method consists of first splitting the differential equation into a stiff and a non-stiff part, respectively, and then following a dynamical low-rank approach. We conduct an error analysis of the proposed procedure, which is independent of the stiffness and robust with respect to possibly small singular values in the approximation matrix. Following the proposed method, we show how to obtain low-rank approximations for differential Lyapunov and for differential Riccati equations. Our theory is illustrated by numerical experiments.

==> integrator.tex <==
% !TEX encoding = UTF-8
% !TEX program = pdflatex
% !TEX root = OPW17.tex

\section{Numerical integrator}

The first subproblem can be solved exactly and it preserves the low-rank structure of the initial value. 
{\color{blue} (Find references for the low-rank treatment of low-rank solution for linear problems and explain better the fact that for linear problems the low-rank manifold does not change).} 
For the low-rank integration of \eqref{sub2} we propose the projector-splitting integrator we have recalled in Section \ref{proj-split}.
{\color{blue} (Stress the fact that the projector-splitting adapts dynamically in time the tangent space but the manifold is set in the beginning with the choice of the approximation rank).}

{\color{blue}
\begin{itemize}
	\item Explain the integrator (mention Leja interpolation for the first subproblem)
	\item Advantage: we split the stiff term away from the non-stiff part
\end{itemize}}




==> motivation.tex <==
% !TEX encoding = UTF-8
% !TEX program = pdflatex
% !TEX root = OPW17.tex

\section{Dynamical low-rank approximation for stiff problems} \label{motivation}
The dynamical low-rank approximation was first considered in \cite{KL07}, which in the field of quantum dynamics is known as the Dirac--Frenkel time-dependent variational principle. The situations of interest are either approximating an explicitly given large data matrix $X(t) \in \C^{m \times n}$ or computing low-rank approximations to the solution of matrix differential equations 
\begin{align}\label{odeX}
	\dot{X}(t) = F(t, X(t)), \qquad X(t_0) = X^0.
\end{align}   
We seek an approximation of $X(t)$ on the manifold $\M$ of rank-$r$ matrices $\M:= \left\{Y(t) \in \C^{m \times n}: \text{rank}(Y(t)) = r \right\}$. We denote by $Y(t)$ a low-rank solution to \eqref{odeX} which is determined by requiring 
\[ \dot{Y}(t) \in \mathcal{T}_{Y}\M, \qquad \lVert \dot{Y}(t) - \dot{X}(t) \rVert = \text{min}, \]
where $\TM$ is the tangent space of the low-rank manifold at the current approximation $Y(t)$. 
Then, an evolution equation for $Y(t)$ is obtained by projecting the right-hand side of \eqref{odeX} orthogonally onto the tangent space. Denoting the orthogonal projection onto the low-rank manifold $\M$ at the current approximation matrix $Y$ by $P(Y)$, we obtain 
\begin{align}\label{odeY}
	\dot{Y}(t) = P(Y)F(t,Y(t)), \qquad Y(t_0) = Y^0,
\end{align}
where $Y^0$ is a low-rank approximation to $X^0$. 
The matrix $Y(t)$ is not computed directly from \eqref{odeY} by applying an integration method. In fact, we make use of its low-rank representation 
\begin{align}\label{svd}
	Y(t) = U(t)S(t)V(t)^*,
\end{align}
where $U(t) \in \C^{m \times r}, V(t) \in \C^{n \times r}$ having orthonormal columns and with invertible $S(t) \in \C^{r \times r}$, which contains the singular values of $Y(t)$. In contrast to the singular value decomposition, this non-unique factorization does not require $S(t)$ to be diagonal. From the computational perspective, this representation has the advantage of a significant reduction in memory requirements and in computational cost if $r \ll m, n$. The time integration is then performed on the low-rank factors.

Moreover, recently, a very efficient integrator for the solution of \eqref{odeY} has been proposed in \cite{LO14}, the so-called projector-splitting integrator. It makes use of the SVD-like representation \eqref{svd} and is based on splitting the projection onto the tangent space of the low-rank manifold.  Now, following \cite[Lemma 4.1]{KL07}, the orthogonal projection $P(Y)$ onto the tangent space $\mathcal{T}_{Y}\M$ at the current approximation matrix $Y = USV\trasp \in \M$ can be written as  
\begin{align*}
\dot{Y}(t) &= UU\trasp F(t,Y) - UU\trasp F(t,Y) VV\trasp + F(t,Y) VV\trasp,
\end{align*}
where $UU\trasp$ and $VV\trasp$ are orthogonal projections onto the spaces spanned by the range and corange of $Y$, respectively.
One time step from $t_0$ to  $t_1=t_0+\tau$ of the first-order integrator consists of solving the following evolution equations consecutively
\begin{align}\label{subodes}
\begin{split}
\dot{Y}_a(t) &= P_a(Y)F(t,Y), \qquad Y_a(t_0) = Y^0, \\
\dot{Y}_b(t) &= -P_b(Y)F(t,Y), \qquad Y_b(t_0) = Y_a(t_1), \\
\dot{Y}_c(t) &= P_c(Y)F(t,Y), \qquad Y_c(t_0) = Y_b(t_1).  
\end{split}
\end{align}
We used the following notation with $B \in \C^{m \times n}$
\[P_a(Y)B = UU\trasp B, \quad P_b(Y)B = UU\trasp B VV\trasp, \quad P_c(Y) B = B VV\trasp. \]
In practice, those differential equations have to be solved using a numerical method, such as a Runge--Kutta method. 

Remarkably, in the case where the matrix $X(t)$ is given explicitly and is of rank-$r$ for all considered times with $X(t_0) = Y^0$, this numerical integrator applied on 
\begin{align}\label{exact}
 \dot{Y}(t) = P(Y)\dot{X}(t), \qquad X(t_0) = Y^0
\end{align}
provides the exact solution for each time step, i.e. $Y^1 = X(t_1)$. This result is proven in \cite[Theorem 4.1]{LO14}. 

Another favorable property of the projector-splitting integrator is its robustness with respect to small singular values. 
A comprehensive error analysis which shows this result is given in \cite{KLW16}. There, the error bounds depend on the Lipschitz constant of $F(t,Y(t))$, among others. This suggests, that the projector-splitting integrator is not applicable to stiff differential equations without being subject to a severe step size restriction. To the contrary, numerical experiments show, that the projector-splitting integrator results in good low-rank approximations also for stiff problems. This phenomenon is not reflected by a rigorous error analysis. Therefore, the objective of the present paper is to give an approach for finding low-rank solutions to nonlinear and stiff differential equations and analyze the error behavior of the method without introducing a Lipschitz condition on $F(t,Y(t))$. 

In the present paper, we restrict to the matrix setting. An important remark is that the dynamical low-rank approximation can also be extended to tensors with different formats, such as tensor trains \cite{LOV15}, Tucker tensors {\color{red}[LVW, in preparation]} or hierarchical tucker tensors \cite{LRSV13}. \\

{\color{red} To do: Numerical example}

